A Survey on the Use of AI and ML for Fighting the COVID-19 Pandemic

Artificial intelligence (AI) and machine learning (ML) have made a paradigm shift in health care which, eventually can be used for decision support and forecasting by exploring the medical data. Recent studies showed that AI and ML can be used to fight against the COVID-19 pandemic. Therefore, the objective of this review study is to summarize the recent AI and ML based studies that have focused to fight against COVID-19 pandemic. From an initial set of 634 articles, a total of 35 articles were finally selected through an extensive inclusion-exclusion process. In our review, we have explored the objectives/aims of the existing studies (i.e., the role of AI/ML in fighting COVID-19 pandemic); context of the study (i.e., study focused to a specific country-context or with a global perspective); type and volume of dataset; methodology, algorithms or techniques adopted in the prediction or diagnosis processes; and mapping the algorithms/techniques with the data type highlighting their prediction/classification accuracy. We particularly focused on the uses of AI/ML in analyzing the pandemic data in order to depict the most recent progress of AI for fighting against COVID-19 and pointed out the potential scope of further research.

==> Conclusion.tex <==
\section{CONCLUSION}

This paper presents a systematic review of exploring AI and ML techniques in fighting the COVID-19 pandemic. A total of 35 research articles were reviewed. These papers are analyzed and compared in various dimensions including the data types, input features, the AI techniques (the machine learning classification algorithms), as well as their objectives. Overall, there are three main contributions of our work. First, we have provided a summary of the findings in terms of objectives, data sources, data type, and volumes. Second, we have explored AI techniques that include various machine learning and deep neural network techniques in the field and compared their outcomes considering several popular evaluation metrics. Finally, we have identified several research issues based on our analysis and introduced corresponding new directions for future research. 

Our study has a number of limitations, but at the same time, it provides some avenues for future research. First, we have used some specific keywords for searching the relevant materials. Although, our search keywords provided effective results to achieve the goal of our study, there might be a risk to miss some important materials that did not emerge from our search queries. Second, we think timely and up-to-date materials related to coronavirus and AI techniques are the key things that we have identified, studied, and summarized in this paper. Therefore, future works would be needed to collect more resources. Third, in addition to exploring AI and ML techniques in fighting the Covid-19 pandemic, future research can be conducted to analyze data privacy and security in the relevant areas. Although we have several limitations mentioned above, our analysis and discussion can have significant implications for both the health practitioners and researchers. We believe that our review opens a promising path and can be used as a reference guide for future research in this area.


==> Introduction.tex <==
\section{INTRODUCTION}
\IEEEPARstart{T}{he} novel and contagious viral pneumonia, COVID-19 (Coronavirus disease-2019) has affected more than 8.2 million people and caused death of more than 440,000 thousand people worldwide. WHO declared it as a global pandemic\cite{who} and suggested that early detection, isolation and prompt treatment can be useful to slow down the COVID-19 outbreak \cite{who2}. Therefore, various bodies have committed themselves to conduct research focusing on COVID-19 to support global response.

With new discoveries being announced at a breathtaking pace, artificial intelligence (AI) has re-emerged into scientific consciousness. AI is a branch of computer science that can be used to build intelligent systems. It is often instantiated as a software program \cite{ligeza}. Recent application of AI in diagnosing disease s has broadened the frontier of AI which once was a humans’ expertise. Medicine and the health care systems are among the most promising areas of application of AI which can be traced back to as early as mid-twentieth century\cite{ai}. Researchers proposed and successfully developed several decision support systems\cite{jamia}. The rule-based system gained success in the late ‘70s\cite{aim} and had been useful in detecting disease\cite{abdominal}, interpreting ECG images\cite{ecg}, choosing appropriate treatment and generate hypothesis by the physicians\cite{inter}. Unlike this first-generation knowledge-based AI system, which relies upon the prior medical knowledge of experts and the formulation based rules, modern AI leverages machine learning algorithms to find pattern and associations in data \cite{circ} \cite{sarker2019effectiveness} \cite{sarker2018mining}. The recent renaissance in AI can be attributed to the successful application of deep learning to a great extent- training an artificial neural network with a large number of labelled datasets. A modern deep learning network usually contains hundreds of hidden layers\cite{nature}. The recent resurgence of AI has been fueling a question of whether AI-doctors will replace human physicians shortly. Yet to be confirmed, researchers believe that AI driven intelligent systems can significantly help human physicians in making better and quick decisions and even sometimes remove the necessity of human decision i.e. radiology\cite{vasc}. The increasing data in health care resulting from increased use of digital technology and the advancement of big data analytics can be attributed to the recent success of AI in healthcare\cite{vasc}. Although AI research in healthcare is emerging, most of the research is concentrated on three diseases: cancer, neurology and cardiology. Guided by evidence, a strong AI can reveal the insight of the medical data which eventually can be used for decision support and forecasting\cite{jama}, \cite{omics}, \cite{ccr}.
 
As AI has been proved useful in healthcare, researchers suggest that it may also be helpful in fighting against COVID-19. From forecasting of a pandemic to designing anti-viral-replication molecules, AI has made a paradigm shift in health care. Recent research on COVID-19 using AI suggests that AI can be helpful in detecting COVID-19 infection, detecting infected population, predicting the next outbreak, finding the attack pattern and even finding a cure \cite{artificial}, \cite{Wang} , \cite{con}. The objective of this review is to explore the existing AI-based research that has been conducted to fight against COVID-19 pandemic. 
The organization of the remaining section is as follows. The methodology to conduct this review study is discussed in section 2. The review data analysis and findings are discussed in detail in section 3. Section 4 presents the main findings and the potential scopes of future research to fight against the COVID-19. Finally, the concluding remark, research limitation and future work are presented in section 5.

